Contrastive Self-Supervised Learning Based Approach for Patient Similarity: A Case Study on Atrial Fibrillation Detection from PPG Signal

In this paper, we propose a novel contrastive learning based deep learning framework for patient similarity search using physiological signals. We use a contrastive learning based approach to learn similar embeddings of patients with similar physiological signal data. We also introduce a number of neighbor selection algorithms to determine the patients with the highest similarity on the generated embeddings. To validate the effectiveness of our framework for measuring patient similarity, we select the detection of Atrial Fibrillation (AF) through photoplethysmography (PPG) signals obtained from smartwatch devices as our case study. We present extensive experimentation of our framework on a dataset of over 170 individuals and compare the performance of our framework with other baseline methods on this dataset.

==> files/abstract.tex <==
% We develop a framework that integrates a model to assess the similarity between patients using their physiological signal data. Initially, we devised a deep learning model to produce embeddings from time series data. Subsequently, we evaluated various neighbor selection algorithms to determine the patients with the highest similarity based on the generated embeddings. We have chosen the detection of Atrial Fibrillation (AF) through photoplethysmography (PPG) signals obtained from a smartwatch device as our case study to validate the effectiveness of our framework for measuring patient similarity.

% % Contrastive Self-Supervised Learning Based Approach for Patient Similarity: A Case Study on Atrial Fibrillation Detection from PPG Signal

==> files/acknowledgement.tex <==
This research has been conducted at DataLab@BUET (\url{datalab.buet.io}).

==> files/performance_test.tex <==
\begin{table*}[hbt]
\begin{center}
\caption{\label{tab:Perf_table_test}Performance of AF detection on the test set from Photoplethysmography data. Lowest performance for each metric is shown in \textcolor{gray}{gray} while the highest performance is \textbf{bolded}}
% \vspace{-2mm}
\begin{tabular}{lccccccc}
    \toprule
     & Sensitivity & Specificity & Precision & F1 & AUC & MCC & Coverage(\%)\\
    \midrule
    \cite{shen2019ambulatory} & \textcolor{gray}{0.664} & 0.819 & 0.706 & 0.684 & 0.806 & 0.489 & 100\\
    % \midrule
    
    \cite{torres2020multi} (\emph{Deepbeat}) & \textbf{0.803} & \textcolor{gray}{0.568} & {0.548} & {0.652} & \textcolor{gray}{0.774} & \textcolor{gray}{0.370} & 100\\
    % \midrule
    \cite{torres2020multi} (\emph{Deepbeat}, Non-poor) & 0.721 & 0.830 & {0.585} & {0.646} & 0.852 & 0.517 & 27.67\\
    % \midrule
    \cite{torres2020multi} (\emph{Deepbeat}, Excellent only) & 0.688 & 0.845 & \textcolor{gray}{0.498} & \textcolor{gray}{0.580} & 0.841 & 0.474 & 18.77\\
    % \midrule
    BayesBeat & 0.722 & 0.72 & 0.627 & 0.671 & 0.793 & 0.433 & 100\\
    % \midrule
    BayesBeat (uncertainty threshold = 0.05) & 0.728 & \textbf{0.892} & \textbf{0.783} & \textbf{0.754} & \textbf{0.858} & \textbf{0.632} & 54\\
    % BayesBeat (uncertainty threshold = 0.01) & 0.736 & \textbf{0.918} & \textbf{0.820} & \textbf{0.776} & \textbf{0.872} & \textbf{0.673} \\
    \bottomrule
\end{tabular}
\end{center}
\end{table*}

==> files/pseudocode.tex <==
\begin{algorithm}[htb]
\footnotesize
\DontPrintSemicolon
  
  \KwIn{parameters, $\theta = (\mu, \rho)$, minibatches, $\mathcal{D} = \{\mathcal{D}_1, \mathcal{D}_2, \ldots, \mathcal{D}_M\}$ number of draws, $n$}
  \KwOut{Updated model parameters, $\theta_{out}$ }
  
  \For{i = $1 \to M$}
    {
     $cost = 0$\\
     $\lambda_i = get\_lambda(i, M)$\\
     \For{k = $1 \to n$}
     {
        Sample $\epsilon \sim \mathcal{N}(0,I)$\\
        $w = \mu + \log [1 + exp(\rho)] \circ \epsilon$\\
        $term_{prior} = \log q(\mathbf{w}^{(k)} | \theta) - \log P(\mathbf{w}^{(k)})$ \hfill (Eq. \ref{eq:cost_approx})\\
        $term_{likelihood} = -\log P(\mathcal{D} | \mathbf{w}^{(k)})$\\
        $cost = cost + \lambda_i term_{prior} + term_{likelihood}$
     
     }
    find the gradients by backpropagating $cost$
    with respect to $\theta$\\
    update parameters $\theta = (\mu, \rho)$ with the computed gradients\\
    }
    $\theta_{out} = \theta$
 
\caption{Training \emph{BayesBeat} with \emph{BBB}}
\label{algo:train_bbb}
\end{algorithm}



